Stable Messenger: Steganography for Message-Concealed Image Generation

In the ever-expanding digital landscape, safeguarding sensitive information remains paramount. This paper delves deep into digital protection, specifically focusing on steganography. While prior research predominantly fixated on individual bit decoding, we address this limitation by introducing ``message accuracy'', a novel metric evaluating the entirety of decoded messages for a more holistic evaluation. In addition, we propose an adaptive universal loss tailored to enhance message accuracy, named Log-Sum-Exponential (LSE) loss, thereby significantly improving the message accuracy of recent approaches. Furthermore, we also introduce a new latent-aware encoding technique in our framework named \Approach, harnessing pretrained Stable Diffusion for advanced steganographic image generation, giving rise to a better trade-off between image quality and message recovery. Throughout experimental results, we have demonstrated the superior performance of the new LSE loss and latent-aware encoding technique. This comprehensive approach marks a significant step in evolving evaluation metrics, refining loss functions, and innovating image concealment techniques, aiming for more robust and dependable information protection.

==> temp/unused.tex <==
% Steganography emerges as an indispensable tool for safeguarding sensitive information amid the ever-expanding exchange of digital content. The ubiquity of digital communication platforms has accentuated the importance of robust steganographic methods that can withstand the challenges posed by the evolving nature of information dissemination. However, a persistent and fundamental challenge remains—the imperative to preserve the entirety of hidden secrets. This imperative holds particular significance for applications ranging from watermarked images, where content integrity is paramount, to real-world steganography scenarios, where the successful concealment of information is contingent upon the fidelity of the hidden content.
% Remarkably, despite the increasing prevalence of steganographic methods, the evaluation frameworks in previous studies \cite{zhu2018hidden, zhang1909rivagan, tancik2020stegastamp, bui2023rosteals} have often overlooked this critical metric of preserving the entire hidden secret. This oversight prompts a reevaluation of existing methodologies and a redefinition of evaluation criteria to align more closely with real-world imperatives. 


% On the one hand, these models are great tools to elevate the power of image watermarking and steganography. 
% They are able to synthesize high-quality images from text prompts and message encoding modules can be integrated inside these networks to produce watermarking and steganography with higher fidelity and imperceptibility. 
% 
